Knowledge boosting during low-latency inference

Models for low-latency, streaming applications could benefit from the knowledge capacity of larger models, but edge devices cannot run these models due to resource constraints. A possible solution is to transfer hints during inference from a large model running remotely to a small model running on-device. However, this incurs a communication delay that breaks real-time requirements and does not guarantee that both models will operate on the same data at the same time. We propose knowledge boosting, a novel technique that allows a large model to operate on time-delayed input during inference, while still boosting small model performance. Using a streaming neural network that processes 8 ms chunks, we evaluate different speech separation and enhancement tasks with communication delays of up to six chunks or 48 ms. Our results show larger gains where the performance gap between the small and large models is wide, demonstrating a promising method for large-small model collaboration for low-latency applications. Code, dataset, and audio samples available at https://knowledgeboosting.cs.washington.edu/.

==> results-1.tex <==
% TODO:
% Add detailed training procedure
% Num epochs, batch size, gradient clip, scheduler


\section{Experiments and Results}
\begin{table}
		\caption{Causal TF-GridNet Hyperparameters}
		\label{tfg-hp}
		\centering
		\begin{tabular}{lll}
			\toprule
%			\multicolumn{2}{c}{Part}                   \\
%			\cmidrule(r){1-2}
			\textbf{Hyperparameter}     & \textbf{Description}   \\
			\midrule
			D & Embedding dimension for each T-F unit   \\
			B     & Number of TF-GridNet blocks    \\
			\midrule
			I     & Kernel size for Unfold and Deconv1D         \\
			J     & Stride size for Unfold and Deconv1D        \\
			H     & Number of hidden units in LSTM \\
			\midrule
			L     & Number of heads in self-attention \\
			\bottomrule
		\end{tabular}
  \end{table}
	

\noindent{\bf Datasets.} To generate binaural audio mixtures, we first sample  rooms from one of 4 binaural room impulse response datasets -- CIPIC~\cite{cipic}, RRBRIR~\cite{rrbrir}, ASH-Listening-Set~\cite{ash-listening}, and CATTRIR~\cite{cattrir} -- with probability 0.35, 0.05, 0.45 and 0.15. We then sample a number of speech utterances from the LibriSpeech~\cite{LibriSpeech} dataset and convolve each of them with a binaural room impulse response from the sampled room. We sum up these binaural speech signals to obtain a binaural speech mixture. For the speech separation and target speaker extraction tasks, the resulting mixture is created from exactly two speech binaural speech utterances. For speech enhancement, we only use a single speech utterance. Moreover, instead of using the room impulse response on a single-channel noise signal, which would only simulate a noise source in a single direction, we use a binaural noise signal recorded in the WHAM!~\cite{wham} dataset as our ambient binaural noise. In this scenario, we scale the noise signal so that the resultant average signal-to-noise ratio across both microphone channels is uniformly distributed in the range $[-6,6]~$dB. For each task, we generate 100k mixtures of training, 5k for testing and 5k for validation. All synthesized audio mixtures are 5 seconds long and the sampling rate is 16~kHz. There is no overlap in the identity of the speakers, the room impulse responses, and noise sources between the train, test and validation splits.\\

\noindent{\bf Loss functions and training hyperparameters.} For the target speaker extraction and speech enhancement tasks, we optimize the network parameters to maximize the average scale-invariant signal-to-distortion ratio (SI-SDR)~\cite{sisdr} across the two microphone channels. In contrast, for speech separation, we output two speaker channels per microphone, and use permutation invariant training to maximize the average SI-SDR across speakers and microphones. In all three tasks, since we are not particularly concerned about binaural cues, we treat the left and right channels independently when computing the optimal scale factor for SI-SDR.

The small and large model baselines are trained for 100 epochs with an initial learning rate of 2e-3. To jointly train our proposed system, we train for 20 epochs starting with an initial learning rate of 1e-3. In each epoch, we iterate over the entire training and validation sets, and halve the learning if the average signal-to-noise ratio (SI-SNR) over the validation set does not decrease after four iterations. For all training runs, we use a batch size of 8 and we use gradient clipping with the norm set to 1.\\

\noindent{\bf Evaluation Setup.} We aim to show that the performance of a small model augmented with delayed hints from a large model during inference time can be significantly greater than the performance of the small model alone. Following~\cite{tfgridnet}, we use the hyper-parameter naming conventions shown in Fig.~\ref{tab:tfg-hp}. In all of the following experiments, we set $I=1, J=1$, chunk size to 128, chunk padding size to 64, and local attention length to 50. We first train the baseline small model for a specific task alone with $D=16, L=4, B=3, H=16$, and no attention. We then train a baseline large model for the same task alone with $D=64, L=8, B=3, H =64$ with attention. 
% TODO: ADD LOOKAHEAD
% ADD NOTE ABOUT TSE TASK (WHAT IS USED TO GENERATE/MERGE EMBEDDINGS?)
For the source separation task, we train the large model and small model jointly as specified in Section~\ref{section:methods}, with a compression ratio $P=1$ as in Table~\ref{table:base-jointSS}, and sweep delays $C = 0, 1, 3, 6$ chunks, corresponding to $0, 8, 24,$ and $48$ ms, respectively. In Table~\ref{table:frozen-jointSS}, we investigate the effects of freezing the large model during training on overall performance, using $P=1$ and sweeping $C = 0, 1, 3, 6$ chunks. Compression of the hints from the large model sent back to the small model allows reductions in bandwidth necessary for transmission(?). In Table~\ref{table:comp-jointSS}, we test compression ratios $P= 1, 2, 4$ for $C = 0, 1, 6$ chunks. Finally, we also sweep $C = 0, 1, 3, 6$ with $P=1$ across speech enhancement (Table~\ref{table:comp-jointSE}) and target speech extraction (Table~\ref{table:jointTSE}) tasks to evaluate the application of knowledge boosting to a variety of tasks.

\noindent{\bf Results.}
% Also maybe include MACs here and parameter count for our modifications??
% How do we justify a fair comparison if the TSE task has way more parameters?
Overall, we observe that knowledge boosting tends to improve the performance of a small model over a small model without knowledge boosting. Based on our evaluations in Table~\ref{table:base-jointSS}, we find that larger $C$ values, or delay values, cause performance to go down, but still generate results that significantly top the performance of the small model alone. From the results in Table~\ref{table:frozen-jointSS}, we find that freezing the large model during training does not lead to optimal performance across our experiments. We also find that compression of the information sent from the large model to the small model (i.e. larger $P$) drops performance across $C$ values by XXX to XXX dB. 
The original size of the small model in our experiments is $23.96$k parameters. Our modifications to introduce the merge method introduce $12.58$k parameters for a final small model size of $36.54$k parameters (but this is only for SS?) Finally, we observe performance increases of XXX-XXX dB and XXX-XXX dB for SE and TSE respectively for $C \in \{0,1,3,6\}$. This leads us to believe that knowledge boosting performs better when the gap between the large and small model baseline performance is larger, and also when the task is more challenging.
% Add intuition as to why TSE improves a lot compared to SE
% SE speech from noise have spectrally different compared to speech and speech
% One from a mix of 2 extract rich speech features which requires model with large number of learned params
% SE beamforming 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TABLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[th]
  \caption{Experiments on SS for different delay configurations with no compression.}
  \label{tab:example}
  \centering
  \begin{tabular}{ c c c c c }
    \toprule
    \multicolumn{1}{c}{\textbf{Config.}} & \multicolumn{1}{c}{\textbf{C}}  &
    \multicolumn{1}{c}{\textbf{SI-SDR}} & \multicolumn{1}{c}{\textbf{PESQ}} &
    \multicolumn{1}{c}{\textbf{STOI}}\\
    \midrule
    Mixture & - & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \midrule
    Small & - & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    Large & - & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \midrule
    BJ-SS & 0 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 1 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 3 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 6 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \midrule
    FJ-SS & 0 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    FJ-SS & 1 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    FJ-SS & 3 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    FJ-SS & 6 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[th]
  \caption{Experiments on SS for different delay configurations with different compression factors.}
  \label{tab:example2}
  \centering
  \begin{tabular}{ c c c c c c }
    \toprule
    \multicolumn{1}{c}{\textbf{Config.}} & \multicolumn{1}{c}{\textbf{C}}  & \multicolumn{1}{c}{\textbf{P}} &
    \multicolumn{1}{c}{\textbf{SI-SDR}} & \multicolumn{1}{c}{\textbf{PESQ}} &
    \multicolumn{1}{c}{\textbf{STOI}}\\
    \midrule
    Mixture & - & - & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \midrule
    Small & - & - & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    Large & - & - & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \midrule
    BJ-SS & 0 & 1 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 1 & 1 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 6 & 1 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \midrule
    BJ-SS & 0 & 2 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 1 & 2 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 6 & 2 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \midrule
    BJ-SS & 0 & 4 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 1 & 4 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 6 & 4 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[th]
  \caption{Experiments on SE for different delay configurations with no compression.}
  \label{tab:example3}
  \centering
  \begin{tabular}{ c c c c c }
    \toprule
    \multicolumn{1}{c}{\textbf{Config.}} & \multicolumn{1}{c}{\textbf{C}}  &
    \multicolumn{1}{c}{\textbf{SI-SDR}} & \multicolumn{1}{c}{\textbf{PESQ}} &
    \multicolumn{1}{c}{\textbf{STOI}}\\
    \midrule
    Mixture & - & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \midrule
    Small & - & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    Large & - & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \midrule
    BJ-SS & 0 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 1 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 3 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 6 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[th]
  \caption{Experiments on TSE for different delay configurations with no compression.}
  \label{tab:example4}
  \centering
  \begin{tabular}{ c c c c c }
    \toprule
    \multicolumn{1}{c}{\textbf{Config.}} & \multicolumn{1}{c}{\textbf{C}}  &
    \multicolumn{1}{c}{\textbf{SI-SDR}} & \multicolumn{1}{c}{\textbf{PESQ}} &
    \multicolumn{1}{c}{\textbf{STOI}}\\
    \midrule
    Mixture & - & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \midrule
    Small & - & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    Large & - & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \midrule
    BJ-SS & 0 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 1 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 3 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    BJ-SS & 6 & 0.00 $\pm$ -0.09 & 8.65 $\pm$-6.52 & 8.65 $\pm$-6.52 \\
    \bottomrule
  \end{tabular}
\end{table}
